Challenges in Migrating Imperative Deep Learning Programs to Graph Execution: An Empirical Study

Efficiency is essential to support responsiveness w.r.t. ever-growing datasets, especially for Deep Learning (DL) systems. DL frameworks have traditionally embraced deferred execution-style DL code that supports symbolic, graph-based Deep Neural Network (DNN) computation. While scalable, such development tends to produce DL code that is error-prone, non-intuitive, and difficult to debug. Consequently, more natural, less error-prone imperative DL frameworks encouraging eager execution have emerged but at the expense of run-time performance. While hybrid approaches aim for the "best of both worlds," the challenges in applying them in the real world are largely unknown. We conduct a data-driven analysis of challenges -- and resultant bugs -- involved in writing reliable yet performant imperative DL code by studying 250 open-source projects, consisting of 19.7 MLOC, along with 470 and 446 manually examined code patches and bug reports, respectively. The results indicate that hybridization: (i) is prone to API misuse, (ii) can result in performance degradation -- the opposite of its intention, and (iii) has limited application due to execution mode incompatibility. We put forth several recommendations, best practices, and anti-patterns for effectively hybridizing imperative DL code, potentially benefiting DL practitioners, API designers, tool developers, and educators.

==> Makefile <==
PAPER=paper
all:
	latexmk -pdf -shell-escape $(PAPER)
automated:
	latexmk -pdf -shell-escape -interaction=nonstopmode $(PAPER)
continuous:
	latexmk -pdf -pvc -shell-escape $(PAPER)
preview: all
	gio open $(PAPER).pdf
clean:
	latexmk -C $(PAPER)
	rm -rf _minted-*
	rm -f *.aux *.log *.bbl *.blg *.dvi *.synctex.gz *.out *.fdb_latexmk \
		*.fls *.nav *.toc *.snm *.spl *.vtc *.pyg *.vrb *.bcf *.run.xml *.tdo \
		*-blx.bib
	rm -rf $(PAPER)
test: automated
	chktex -xH -n 6 $(PAPER).tex 2> /dev/null | tee lint.out
	test ! -s lint.out
	! grep -n ' $$' *.tex
html: all
	rm -rf $(PAPER)/
	latex2html -split 0 $(PAPER)
	gio open $(PAPER)/index.html
TODO:
	pandoc -s --metadata title="TODOs" TODO.md -o TODO.html
preview-TODO: TODO
	gio open TODO.html
install-arxiv-latex-cleaner:
	pip install arxiv-latex-cleaner
arXiv: install-arxiv-latex-cleaner
	scripts/prep_arXiv.sh


==> findings.tex <==
\begin{figure}[t]
    \small
    \begin{findings}


    \end{findings}
    \caption{Study findings.}\label{fig:findings}
\end{figure}

